A mmWave Bridge Concept to Solve the Cellular Outdoor-to-Indoor Challenge

Wireless indoor coverage and data capacity are important aspects of cellular networks. With the ever-increasing data traffic, demand for more data capacity indoors is also growing. The lower frequencies of the legacy frequency bands of macro outdoor cells manage to provide coverage inside buildings, however, new frequencies foreseen for the 5th generation (5G) of mobile communications in the millimeter wave (mmWave) spectrum penetrate very poorly into buildings. Therefore, a massive densification of the network would require to deploy a large number of indoor small cells, which would lead to high deployment costs to install the necessary wired/optical backhaul. Hence, other methods are needed that allow an increase of the data capacity indoors, bearing a lower cost than a fiber deployment. We propose a cost-efficient out-of-band repeater architecture that provides more data capacity indoors than an outdoor macro/micro network can provide to indoor, without adversely affecting a legacy network, and which readily works with the established cellular infrastructure as well as standard handsets/smartphones. This proposal is compared to conventional in- and out-of-band repeaters and relay nodes in order to highlight the advantages of our solution. While the data capacity for a single link is similar to that of repeaters and relays, a macro cell can be effectively offloaded. Cell capacities corresponding to at least 3--4 times that of a repeater or relay solution can be provided, depending on the number of parallel installed links and the bandwidth in the mmWave spectrum.

==> results.tex <==
%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
%!!!       NOT USED ANYMORE      !!!
%!!! TO BE REMOVED IN THE FUTURE !!!
%!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!!
\section{Case Study Results}
\label{sec:simuresults}
For the case studies, we present results a rural, suburban, and urban environment, as further described in \cite{Schumacher_3.5GHzCoverageAssessment_2019}. We used the 3GPP path loss models that matched best according to the aforementioned paper: \emph{Rural Macro} (RMa) for the rural and suburban environment, \emph{Urban Macro} (UMa) for the urban environment. However, to match the calculated outdoor SNR with the measured outdoor SNR at LOS locations, the path loss for LOS had to be corrected by adding $10 \log_{10}(8.78\cdot10^{-9}\cdot f_c)$. For these studies we do not consider neighboring cells and thus neglect such interference. But, for the study of each concept, we assume that the same frequencies used indoors are radiated outdoors from the same base station (either it is the same serving cell, or for the mmWave bridge, layer~3 relay, and small cell, a frequency independently used outdoors).

The simulations have been based on the population density per hectare (100$\times$100\,m)\footnote{Swiss Federal Statistical Office, \url{https://www.bfs.admin.ch}} and the digital height model DHMS25/200\footnote{Swiss Federal Office of Topography, \url{https://www.swisstopo.ch}}.

\subsection{Coverage}

For the sake of brevity, we skip the plots showing the estimated outdoor received power, and instead directly show the estimated outdoor SNR for all environments for the four carrier frequencies under study. See \fref{fig:SNRmapRural} for the rural, \fref{fig:SNRmapSuburban} for the suburban, and \fref{fig:SNRmapUrban} for the urban environment. Note that the SNR depends on the power density, therefor also the respective carrier bandwidth is given in the figure captions. However, the coverage is usually limited by the UL due to the lower transmit power on the UE side. Considering a minimum SINR of -4.9\,dB in the gNB UL receiver and the noise figure from \tref{tab:simu_params}, we can estimate the maximum distance for which an UL transmission can still work. In the three cases, there are only limitations for the mmWave bands. The maximum link distances for the rural, suburban, and urban cases are 350\,m, 600\,m, 250\,m, respectively (light gray arcs around the base station in Figs.~\ref{fig:SNRmapRural}--\ref{fig:SNRmapUrban}).

\begin{figure}
	\centering
	%\vspace{-1em}
	\subfloat[$f_c$ = 1.8\,GHz, $B$ = 20\,MHz, \newline $P_{\text{tx}}$ = 1000\,W ERP\label{fig:SNRmap1800rural}\vspace{-1em}]{%
		\includegraphics[width=0.49\linewidth]{SINR_Map_rural_1800MHz}}
	\hfill
	\subfloat[$f_c$ = 3.6\,GHz, $B$ = 100\,MHz, \newline $P_{\text{tx}}$ = 1000\,W ERP\label{fig:SNRmap3600rural}\vspace{-1em}]{%
		\includegraphics[width=0.49\linewidth]{SINR_Map_rural_3600MHz}}
	\\
	\subfloat[$f_c$ = 26\,GHz, $B$ = 400\,MHz, \newline $P_{\text{tx}}$ = 1500\,W ERP\label{fig:SNRmap26rural}]{%
		\includegraphics[width=0.49\linewidth]{SINR_Map_rural_26000MHz}}
	\hfill
	\subfloat[$f_c$ = 39\,GHz, $B$ = 400\,MHz, \newline $P_{\text{tx}}$ = 1500\,W ERP\label{fig:SNRmap39rural}]{%
		\includegraphics[width=0.49\linewidth]{SINR_Map_rural_39000MHz}}
	\caption{SNR coverage for a rural environment for the frequencies 1.8\,GHz (a), 3.6\,GHz (b), 26\,GHz (c), 39\,GHz (d).
	\label{fig:SNRmapRural}}
\end{figure}
%\begin{mysubfigure}
%	\raggedbottom% esthetics
%	\begin{subfigure}{0.48\columnwidth}
%		\centering
%		\includegraphics[width=0.49\linewidth]{SINR_Map_rural_1800MHz}
%		\caption{$f_c$ = 1.8\,GHz, $B$ = 20\,MHz, \newline $P_{\text{tx}}$ = 1000\,W ERP\label{fig:SNRmap1800rural}\vspace{-1em}}
%	\end{subfigure}
%	\begin{subfigure}{0.48\columnwidth}
%		\centering
%		\includegraphics[width=0.49\linewidth]{SINR_Map_rural_3600MHz}
%		\caption{$f_c$ = 3.6\,GHz, $B$ = 100\,MHz, \newline $P_{\text{tx}}$ = 1000\,W ERP\label{fig:SNRmap3600rural}\vspace{-1em}}
%	\end{subfigure}
%	\begin{subfigure}{0.49\linewidth}
%		\centering
%		\includegraphics[width=0.49\linewidth]{SINR_Map_rural_26000MHz}
%		\caption{$f_c$ = 26\,GHz, $B$ = 400\,MHz, \newline $P_{\text{tx}}$ = 1500\,W ERP\label{fig:SNRmap26rural}}
%	\end{subfigure}
%	\begin{subfigure}{0.49\linewidth}
%		\centering
%		\includegraphics[width=0.49\linewidth]{SINR_Map_rural_39000MHz}
%		\caption{$f_c$ = 39\,GHz, $B$ = 400\,MHz, \newline $P_{\text{tx}}$ = 1500\,W ERP\label{fig:SNRmap39rural}}
%	\end{subfigure}
%	\caption{SNR coverage for a rural environment for the frequencies 1.8\,GHz (a), 3.6\,GHz (b), 26\,GHz (c), 39\,GHz (d).
%		\label{fig:SNRmapRural}}
%\end{mysubfigure}


\begin{figure}
	\centering
	%\vspace{-0.47em}
	\subfloat[$f_c$ = 1.8\,GHz, $B$ = 20\,MHz, \newline $P_{\text{tx}}$ = 500\,W ERP\label{fig:SNRmap1800suburb}\vspace{-1em}]{%
		\includegraphics[width=0.49\linewidth]{SINR_Map_suburban_1800MHz}}
	\hfill
	\subfloat[$f_c$ = 3.6\,GHz, $B$ = 100\,MHz, \newline $P_{\text{tx}}$ = 500\,W ERP\label{fig:SNRmap3600suburb}\vspace{-1em}]{%
		\includegraphics[width=0.49\linewidth]{SINR_Map_suburban_3600MHz}}
	\\
	\subfloat[$f_c$ = 26\,GHz, $B$ = 400\,MHz, \newline $P_{\text{tx}}$ = 500\,W ERP\label{fig:SNRmap26suburb}]{%
		\includegraphics[width=0.49\linewidth]{SINR_Map_suburban_26000MHz}}
	\hfill
	\subfloat[$f_c$ = 39\,GHz, $B$ = 400\,MHz, \newline $P_{\text{tx}}$ = 500\,W ERP\label{fig:SNRmap39suburb}]{%
		\includegraphics[width=0.49\linewidth]{SINR_Map_suburban_39000MHz}}
	\caption{SNR coverage for a suburban environment for the frequencies 1.8\,GHz (a), 3.6\,GHz (b), 26\,GHz (c), 39\,GHz (d).
	\label{fig:SNRmapSuburban}}
\end{figure}

\begin{figure}
	\centering
	%\vspace{-1em}
	\subfloat[$f_c$ = 1.8\,GHz, $B$ = 20\,MHz, \newline $P_{\text{tx}}$ = 300\,W ERP\label{fig:SNRmap1800urban}\vspace{-1em}]{%
		\includegraphics[width=0.49\linewidth]{SINR_Map_urban_1800MHz}}
	\hfill
	\subfloat[$f_c$ = 3.6\,GHz, $B$ = 100\,MHz, \newline $P_{\text{tx}}$ = 300\,W ERP\label{fig:SNRmap3600urban}\vspace{-1em}]{%
		\includegraphics[width=0.49\linewidth]{SINR_Map_urban_3600MHz}}
	\\
	\subfloat[$f_c$ = 26\,GHz, $B$ = 400\,MHz, \newline $P_{\text{tx}}$ = 200\,W ERP\label{fig:SNRmap26urban}]{%
		\includegraphics[width=0.49\linewidth]{SINR_Map_urban_26000MHz}}
	\hfill
	\subfloat[$f_c$ = 39\,GHz, $B$ = 400\,MHz, \newline $P_{\text{tx}}$ = 200\,W ERP\label{fig:SNRmap39urban}]{%
		\includegraphics[width=0.49\linewidth]{SINR_Map_urban_39000MHz}}
	\caption{SNR coverage for a urban environment for the frequencies 1.8\,GHz (a), 3.6\,GHz (b), 26\,GHz (c), 39\,GHz (d).
	\label{fig:SNRmapUrban}}
\end{figure}


\subsection{Capacity}

Based on the SINR for the DL and UL, the capacity can be computed. As explained in \sref{sec:capacity}, the capacity is adjusted with the TDD DL to UL ratio of 4:1. If the UL SINR is too low for a communication link, this of course also cuts the DL.
The median indoor DL capacities for each frequency and concept are listed in \tref{tab:capa_res} for the rural, suburban, and urban environment.
%The median indoor DL capacities for each frequency and concept are listed in \tref{tab:capa_res_rural}, \tref{tab:capa_res_suburb}, and \tref{tab:capa_res_urban}, for the rural, suburban, and urban environment, respectively.

% For heatmap tables
\newcommand*{\MinNumber}{16.5}%
\newcommand*{\MaxNumber}{1722}%
\newcolumntype{R}{>{\raggedleft\arraybackslash}X}
\newcolumntype{C}{>{\centering\arraybackslash}X}
\newcolumntype{L}{>{\raggedright\arraybackslash}X}

%\def\cca#1{%
%%	\pgfmathsetmacro\calc{(ln(#1)-ln(\MinNumber))/(ln(\MaxNumber)-ln(\MinNumber))*70}%
%%	\edef\clrmacro{\noexpand\cellcolor{blue!\calc}}%
%	\newcommand{\calc}{\fpeval{(ln(#1)-ln(\MinNumber))/(ln(\MaxNumber)-ln(\MinNumber))*70}}
%	\edef\clrmacro{\noexpand\cellcolor{blue!\calc}}%
%	\clrmacro%
%	{#1}%
%%	\ifdim \calc pt>60pt\leavevmode\color{white}\fi{#1}%
%}
%
%\begin{table}
%	\centering
%	\caption{Median Indoor SISO DL Capacity in a Rural Environment.
%		M:~Macro; L1R: Layer~1 Repeater; B26/B39: Bridge at 26\,GHz/39\,GHz; SC: Small~Cell; L3R: Layer~3 Relay}
%	\label{tab:capa_res_rural}
%	{\setlength{\tabcolsep}{0pt}
%		\begin{tabularx}{\linewidth}{@{}lCCCCC|CCCC@{}}
%			\toprule
%			In-/Outdoor & M & L1R & B26 & B39 & SC & \multicolumn{4}{c}{L3R: Outdoor Freq. [GHz]} \\
%			Frequency & & & & & & 1.8 & 3.6 & 26 & 39 \\
%			\midrule
%			1.8\,GHz & \cca{51.2} & \cca{116.8} & \cca{116.8} & \cca{116.6} & \cca{116.8} & \cca{116.8} & \cca{116.8} & \cca{116.8} & 0 \\
%			3.6\,GHz & \cca{116.6} & \cca{467.2} & \cca{465.3} & \cca{436.4} & \cca{467.2} & \cca{116.8} & \cca{452.7} & \cca{467.2} & 0 \\
%			26\,GHz & 0 & \cca{1109} & N/A & N/A & \cca{1722} & \cca{116.8} & \cca{452.7} & \cca{985.6} & 0 \\
%			39\,GHz & 0 & 0 & N/A & N/A & \cca{1722} & \cca{116.8} & \cca{452.7} & \cca{985.6} & 0 \\
%			\bottomrule
%\end{tabularx}}
%\end{table}
%
%\begin{table}
%	\centering
%	\caption{Median Indoor SISO DL Capacity in a Suburban Environment.
%	M:~Macro; L1R: Layer~1 Repeater; B26/B39: Bridge at 26\,GHz/39\,GHz; SC: Small~Cell; L3R: Layer~3 Relay}
%	\label{tab:capa_res_suburb}
%	{\setlength{\tabcolsep}{0pt}
%		\begin{tabularx}{\linewidth}{@{}lCCCCC|CCCC@{}}
%			\toprule
%			In-/Outdoor & M & L1R & B26 & B39 & SC & \multicolumn{4}{c}{L3R: Outdoor Freq. [GHz]} \\
%			Frequency & & & & & & 1.8 & 3.6 & 26 & 39 \\
%			\midrule
%			1.8\,GHz & \cca{50} & \cca{116.8} & \cca{116.8} & \cca{115.4} & \cca{116.8} & \cca{116.8} & \cca{116.8} & \cca{116.8} & \cca{116.8} \\
%			3.6\,GHz & \cca{57} & \cca{467.2} & \cca{460.1} & \cca{402.7} & \cca{467.2} & \cca{116.8} & \cca{378} & \cca{467.2} & \cca{467.2} \\
%			26\,GHz & 0 & \cca{1070} & N/A & N/A & \cca{1722} & \cca{116.8} & \cca{378} & \cca{890.4} & \cca{601.9} \\
%			39\,GHz & 0 & \cca{730.6} & N/A & N/A & \cca{1722} & \cca{116.8} & \cca{378} & \cca{890.4} & \cca{601.9} \\
%			\bottomrule
%	\end{tabularx}}
%\end{table}
%
%\begin{table}
%	\centering
%	\caption{Median Indoor SISO DL Capacity in an Urban Environment.
%	M:~Macro; L1R: Layer~1 Repeater; B26/B39: Bridge at 26\,GHz/39\,GHz; SC: Small~Cell; L3R: Layer~3 Relay}
%	\label{tab:capa_res_urban}
%	{\setlength{\tabcolsep}{0pt}
%		\begin{tabularx}{\linewidth}{@{}lCCCCC|CCCC@{}}
%			\toprule
%			In-/Outdoor & M & L1R & B26 & B39 & SC & \multicolumn{4}{c}{L3R: Outdoor Freq. [GHz]} \\
%			Frequency & & & & & & 1.8 & 3.6 & 26 & 39 \\
%			\midrule
%			1.8\,GHz & \cca{16.5} & \cca{116.8} & \cca{110} & \cca{96.3} & \cca{116.8} & \cca{112.7} & \cca{116.8} & \cca{116.8} & \cca{116.8} \\
%			3.6\,GHz & 0 & \cca{463.4} & \cca{361.8} & \cca{299.1} & \cca{467.2} & \cca{112.7} & \cca{258.8} & \cca{467.2} & \cca{307.5} \\
%			26\,GHz & 0 & \cca{791.2} & N/A & N/A & \cca{1722} & \cca{112.7} & \cca{258.8} & \cca{476} & \cca{307.5} \\
%			39\,GHz & 0 & \cca{439.8} & N/A & N/A & \cca{1722} & \cca{112.7} & \cca{258.8} & \cca{476} & \cca{307.5} \\
%			\bottomrule
%	\end{tabularx}}
%\end{table}

\newlength{\vlinewidth}
\setlength{\vlinewidth}{\baselineskip}
\def\cca#1{%
	\newcommand{\calc}{\fpeval{(ln(#1)-ln(\MinNumber))/(ln(\MaxNumber)-ln(\MinNumber))*50}}
	\edef\clrmacro{\noexpand\cellcolor{blue!\calc}}%
	\clrmacro%
	{#1}%
}
\begin{table}
	\centering
	\caption{Median Indoor SISO DL Capacity. M:~Macro Network Baseline; L1R:~Layer~1 Repeater; B26/B39:  Bridge at 26\,GHz/39\,GHz; SC:~Small~Cell; L3R:~Layer~3 Relay}
	\label{tab:capa_res}
	{\setlength{\tabcolsep}{0pt}
		\begin{tabularx}{\linewidth}{@{}llCCCCC|CCCC@{}}
			\toprule
			\multicolumn{2}{l}{In-/Outdoor} & M & L1R & B26 & B39 & SC & \multicolumn{4}{c}{L3R: Outdoor Freq. [GHz]} \\
			\multicolumn{2}{l}{Frequency} & & & & & & 1.8 & 3.6 & 26 & 39 \\
			\midrule
			%& \multicolumn{10}{l}{\emph{Rural Environment}} \\
			\parbox[t]{\vlinewidth}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Rural}}}
			& 1.8\,GHz & \cca{51.2} & \cca{116.8} & \cca{116.8} & \cca{116.6} & \cca{116.8} & \cca{116.8} & \cca{116.8} & \cca{116.8} & 0 \\
			& 3.6\,GHz & \cca{116.6} & \cca{467.2} & \cca{465.3} & \cca{436.4} & \cca{467.2} & \cca{116.8} & \cca{452.7} & \cca{467.2} & 0 \\
			& 26\,GHz & 0 & \cca{1109} & N/A & N/A & \cca{1722} & \cca{116.8} & \cca{452.7} & \cca{985.6} & 0 \\
			& 39\,GHz & 0 & 0 & N/A & N/A & \cca{1722} & \cca{116.8} & \cca{452.7} & \cca{985.6} & 0 \\
			\midrule
			%& \multicolumn{10}{l}{\emph{Suburban Environment}} \\
			\parbox[t]{\vlinewidth}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Suburban}}}
			& 1.8\,GHz & \cca{50} & \cca{116.8} & \cca{116.8} & \cca{115.4} & \cca{116.8} & \cca{116.8} & \cca{116.8} & \cca{116.8} & \cca{116.8} \\
			& 3.6\,GHz & \cca{57} & \cca{467.2} & \cca{460.1} & \cca{402.7} & \cca{467.2} & \cca{116.8} & \cca{378} & \cca{467.2} & \cca{467.2} \\
			& 26\,GHz & 0 & \cca{1070} & N/A & N/A & \cca{1722} & \cca{116.8} & \cca{378} & \cca{890.4} & \cca{601.9} \\
			& 39\,GHz & 0 & \cca{730.6} & N/A & N/A & \cca{1722} & \cca{116.8} & \cca{378} & \cca{890.4} & \cca{601.9} \\
			\midrule
			%& \multicolumn{10}{l}{\emph{Urban Environment}} \\
			\parbox[t]{\vlinewidth}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Urban}}}
			& 1.8\,GHz & \cca{16.5} & \cca{116.8} & \cca{110} & \cca{96.3} & \cca{116.8} & \cca{112.7} & \cca{116.8} & \cca{116.8} & \cca{116.8} \\
			& 3.6\,GHz & 0 & \cca{463.4} & \cca{361.8} & \cca{299.1} & \cca{467.2} & \cca{112.7} & \cca{258.8} & \cca{467.2} & \cca{307.5} \\
			& 26\,GHz & 0 & \cca{791.2} & N/A & N/A & \cca{1722} & \cca{112.7} & \cca{258.8} & \cca{476} & \cca{307.5} \\
			& 39\,GHz & 0 & \cca{439.8} & N/A & N/A & \cca{1722} & \cca{112.7} & \cca{258.8} & \cca{476} & \cca{307.5} \\
			\bottomrule
	\end{tabularx}}
\end{table}


As it can be expected, the baseline without additional equipment (column M) only provides relatively small capacities for sub-6\,GHz bands, and does not provide anything for mmWave bands. Also, the largest capacities can be achieved with indoor small cells (column SC). In-between, the repeater/relay nodes manage to provide decent capacities. It can be noted, that the layer~1 repeater (column L1R) slightly outperforms a layer~3 relay (columns L3R), but only if the signal delay through the layer~1 repeater stays below the cyclic prefix length of the 5G NR and no ISI is created. Since a layer~3 relay not only has a much longer delay, it also creates its own cell. Thus, the outdoor cell signal interferes with the layer~3 relay cell signal, slightly lowering the available capacity.

The mmWave bridge manages to provide almost as much capacity as e.g., an in-band layer~1 repeater. However, the large advantage of the mmWave bridge comes with the frequency and spatial multiplexing that is achieved in mmWave with the large bandwidth and very directional antennas. Assuming a beam width of 10$^\circ$ (see beam sectors indicated with light gray radial lines in Figs.~\ref{fig:SNRmapRural}--\ref{fig:SNRmapUrban}), a high number of beams can concurrently be used with mmWave bridges. A conventional 5G NR cell can only serve up to eight layers, which results in four UEs if each UE uses 2$\times$2 MIMO (two layers).
This is reflected in the estimated peak DL cell capacity listed in \tref{tab:cell_capa_res} for the rural, suburban, and urban environment.
%This is reflected in the estimated peak DL cell capacity listed in \tref{tab:cell_capa_res_rural}, \tref{tab:cell_capa_res_suburb}, and \tref{tab:cell_capa_res_urban}, for the rural, suburban, and urban environment, respectively.

\newcommand*{\MinNumberB}{390}%
\newcommand*{\MaxNumberB}{8000}%

\def\cca#1{%
	\newcommand{\calc}{\fpeval{(ln(#1)-ln(\MinNumberB))/(ln(\MaxNumberB)-ln(\MinNumberB))*70}}
	\edef\clrmacro{\noexpand\cellcolor{green!\calc}}%
	\clrmacro%
	{#1}%
}
%\begin{table}
%	\centering
%	\caption{Peak DL Cell Capacity for Several Concepts (Rural)}
%	\label{tab:cell_capa_res_rural}
%	{\setlength{\tabcolsep}{0pt}
%		\begin{tabularx}{\linewidth}{@{}lCCCCC@{}}
%			\toprule
%			Frequency & Macro & L1 Relay & Bridge26 & Bridge39 & L3 Relay \\
%			\midrule
%			1.8\,GHz & \cca{466} & \cca{467} & \cca{1402} & \cca{1393} & \cca{467} \\
%			3.6\,GHz & \cca{1475} & \cca{1869} & \cca{5606} & \cca{5490} & \cca{1869} \\
%			26\,GHz & 0 & \cca{4885} & N/A & N/A & \cca{4934} \\
%			39\,GHz & 0 & \cca{4680} & N/A & N/A & \cca{4934} \\
%			\bottomrule
%	\end{tabularx}}
%\end{table}
%
%\begin{table}
%	\centering
%	\caption{Peak DL Cell Capacity for Several Concepts (Suburban)}
%	\label{tab:cell_capa_res_suburb}
%	{\setlength{\tabcolsep}{0pt}
%		\begin{tabularx}{\linewidth}{@{}lCCCCC@{}}
%			\toprule
%			Frequency & Macro & L1 Relay & Bridge26 & Bridge39 & L3 Relay \\
%			\midrule
%			1.8\,GHz & \cca{429} & \cca{467} & \cca{1986} & \cca{1947} & \cca{467} \\
%			3.6\,GHz & \cca{1196} & \cca{1869} & \cca{7942} & \cca{7558} & \cca{1869} \\
%			26\,GHz & 0 & \cca{4891} & N/A & N/A & \cca{4934} \\
%			39\,GHz & 0 & \cca{4695} & N/A & N/A & \cca{4932} \\
%			\bottomrule
%	\end{tabularx}}
%\end{table}
%
%\begin{table}
%	\centering
%	\caption{Peak DL Cell Capacity for Several Concepts (Urban)}
%	\label{tab:cell_capa_res_urban}
%	{\setlength{\tabcolsep}{0pt}
%		\begin{tabularx}{\linewidth}{@{}lCCCCC@{}}
%			\toprule
%			Frequency & Macro & L1 Relay & Bridge26 & Bridge39 & L3 Relay \\
%			\midrule
%			1.8\,GHz & \cca{391} & \cca{467} & \cca{1518} & \cca{1419} & \cca{467} \\
%			3.6\,GHz & \cca{1223} & \cca{1869} & \cca{6074} & \cca{5115} & \cca{1843} \\
%			26\,GHz & 0 & \cca{4737} & N/A & N/A & \cca{4640} \\
%			39\,GHz & 0 & \cca{4186} & N/A & N/A & \cca{4151} \\
%			\bottomrule
%	\end{tabularx}}
%\end{table}

\begin{table}
	\centering
	\caption{Peak DL Cell Capacity for Several Concepts}
	\label{tab:cell_capa_res}
	{\setlength{\tabcolsep}{0pt}
		\begin{tabularx}{\linewidth}{@{}llCCCCC@{}}
			\toprule
			\multicolumn{2}{l}{Frequency} & Macro & L1 Relay & Bridge26 & Bridge39 & L3 Relay \\
			\midrule
			%& \multicolumn{6}{l}{\emph{Rural Environment}} \\
			\parbox[t]{\vlinewidth}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Rural}}}
			& 1.8\,GHz & \cca{466} & \cca{467} & \cca{1402} & \cca{1393} & \cca{467} \\
			& 3.6\,GHz & \cca{1475} & \cca{1869} & \cca{5606} & \cca{5490} & \cca{1869} \\
			& 26\,GHz & 0 & \cca{4885} & N/A & N/A & \cca{4934} \\
			& 39\,GHz & 0 & \cca{4680} & N/A & N/A & \cca{4934} \\
			\midrule
			%& \multicolumn{6}{l}{\emph{Suburban Environment}} \\
			\parbox[t]{\vlinewidth}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Suburban}}}
			& 1.8\,GHz & \cca{429} & \cca{467} & \cca{1986} & \cca{1947} & \cca{467} \\
			& 3.6\,GHz & \cca{1196} & \cca{1869} & \cca{7942} & \cca{7558} & \cca{1869} \\
			& 26\,GHz & 0 & \cca{4891} & N/A & N/A & \cca{4934} \\
			& 39\,GHz & 0 & \cca{4695} & N/A & N/A & \cca{4932} \\
			\midrule
			%& \multicolumn{6}{l}{\emph{Urban Environment}} \\
			\parbox[t]{\vlinewidth}{\multirow{4}{*}{\rotatebox[origin=c]{90}{Urban}}}
			& 1.8\,GHz & \cca{391} & \cca{467} & \cca{1518} & \cca{1419} & \cca{467} \\
			& 3.6\,GHz & \cca{1223} & \cca{1869} & \cca{6074} & \cca{5115} & \cca{1843} \\
			& 26\,GHz & 0 & \cca{4737} & N/A & N/A & \cca{4640} \\
			& 39\,GHz & 0 & \cca{4186} & N/A & N/A & \cca{4151} \\
			\bottomrule
	\end{tabularx}}
\end{table}



